ST-Align: A Multimodal Foundation Model for Image-Gene Alignment in Spatial Transcriptomics

Spatial transcriptomics (ST) provides high-resolution pathological images and whole-transcriptomic expression profiles at individual spots across whole-slide scales. This setting makes it an ideal data source to develop multimodal foundation models. Although recent studies attempted to fine-tune visual encoders with trainable gene encoders based on spot-level, the absence of a wider slide perspective and spatial intrinsic relationships limits their ability to capture ST-specific insights effectively. Here, we introduce ST-Align, the first foundation model designed for ST that deeply aligns image-gene pairs by incorporating spatial context, effectively bridging pathological imaging with genomic features. We design a novel pretraining framework with a three-target alignment strategy for ST-Align, enabling (1) multi-scale alignment across image-gene pairs, capturing both spot- and niche-level contexts for a comprehensive perspective, and (2) cross-level alignment of multimodal insights, connecting localized cellular characteristics and broader tissue architecture. Additionally, ST-Align employs specialized encoders tailored to distinct ST contexts, followed by an Attention-Based Fusion Network (ABFN) for enhanced multimodal fusion, effectively merging domain-shared knowledge with ST-specific insights from both pathological and genomic data. We pre-trained ST-Align on 1.3 million spot-niche pairs and evaluated its performance through two downstream tasks across six datasets, demonstrating superior zero-shot and few-shot capabilities. ST-Align highlights the potential for reducing the cost of ST and providing valuable insights into the distinction of critical compositions within human tissue.

==> sec/2_formatting.tex <==
\section{Related Works}
\label{sec:formatting}

%-------------------------------------------------------------------------
\subsection{Multimodal Learning for WSI and Transcriptome}

Previous studies have highlighted the homogeneous and heterogeneous characteristics between WSI and transcriptome, contributing to a comprehensive understanding of patient and cellular statuses. 
Recently, multimodal learning approaches have been developed to embed these data types into a shared feature space and relate them to downstream tasks. 
For instance, PIBD \cite{zhangprototypical} leverages Prototypical Information Disentanglement to decouple specific and common information. 
SurvPath \cite{jaume2024modeling} employs tokenizers and efficient multimodal transformers to fuse WSI with transcriptome data at the pathway level. 
SurvMamba \cite{chen2024survmamba} utilizes the Mamba architecture to capture fine- and coarse-grained transcriptome and pathological knowledge. 
PathAsst \cite{sun2024pathasst} leverages CLIP, trained on large text-image paired datasets, to efficiently synthesize pathological reports. 
Despite their efficiency, existing architectures often treat the integration of WSI and transcriptome data as a MIL problem, given that WSI are vast while transcriptome data is typically gathered at the patient level. Spatial transcriptomic (ST) data, captured at the spot level, provides more fine-grained information on cellular morphology and genomic status, necessitating an innovative workflow.

%-------------------------------------------------------------------------
\subsection{Foundation Models for WSI and Genomic}

Recent advancements in foundation models for WSI and transcriptome data are inspiring. 
In WSI, models like UNI \cite{chen2024towards} and TORCH \cite{tian2024prediction} were pre-trained on millions of WSIs using Vision Transformers (ViT) and self-supervised learning (SSL), performing well on multiple downstream tasks, including risk prediction at the patient level and tissue region classification at the regions of interest (ROIs) level. 
Additionally, CONCH \cite{lu2024visual}, trained on vision-text paired datasets, contributes diverse tissues and diseases classification. 
In the transcriptomic domain, models like scGPT \cite{cui2024scgpt} and scFoundation \cite{hao2024large} were pre-trained on millions of cells, aiding in biology-specific tasks such as cell clustering and drug perturbation prediction. 
LangCell \cite{zhao2024langcell} and CellLM \cite{zhao2023large} integrate transcriptome expression value and text describing each cell's meta-information for training. 
TANGLE \cite{jaume2024transcriptomics} uses the MIL strategy and SSL to train WSI- and transcriptome- specific encoders, excelling in cancer subtype classification. 
However, a specific vision-genomic foundational model to capture the shared and distinct features between WSI and transcriptome data in fine-grained is still lacking.

%-------------------------------------------------------------------------
\subsection{Vision-Genomic Paired Datasets}

Numerous WSI-transcriptome paired datasets have emerged, facilitating the construction of advanced foundational models and providing insightful discoveries. 
For instance, TCGA and GEO offer more than 10,000 vision-genomic paired datasets derived from over 30 human organs. Despite this, these datasets often provide full-resolution WSI paired with transcriptome expression vectors for each patient, limiting the understanding of the relationship between morphology and genetic status at the tissue or cellular level. 
The advancement of ST has facilitated the discovery of spatial dynamics at the cellular level. Public datasets such as 10x Genomics, CROST \cite{wang2024crost}, SODB \cite{yuan2023sodb}, STOmicsDB \cite{xu2024stomicsdb}, and Aquila \cite{zheng2023aquila} collect thousands of spatial multi-omics datasets, enabling comprehensive spatial-level investigation. 
However, most of these data sources are based on multiple diseases, organs, and even species. Currently, there is a lack of datasets specific to human diseases that provide paired image and gene expression data, crucial for bridging the gap between visual information and underlying transcriptome profiles.

%-------------------------------------------------------------------------
\subsection{Benchmark Tasks}

The downstream tasks for WSIs can broadly be categorized into patient- and ROI-level tasks. 
Patient-level tasks include survival or recurrence prediction \cite{chen2024survmamba} and unknown tumor origin tracking \cite{tian2024prediction}, while ROI-level tasks often help to segment regions of interest \cite{chen2024towards}. 
In the context of ST, tasks can be roughly grouped into patient-level, cellular-level, and gene-level. Patient-level tasks include tracking cancer of unknown primary origin \cite{xie2024tracing}, cellular-level tasks involve identifying important cell subpopulations \cite{tong2023prioritizing}, and gene-level tasks focus on denoising gene expression \cite{wang2022sprod}. 
To evaluate the performance of \textbf{ST-Align}, we employed tasks spanning from cellular to genetic levels, specifically focusing on spatial structure identification and missing gene imputation.

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/table1.tex <==
\begin{table*}[ht]
\centering

\caption{\textbf{Performance of different foundation model embeddings in spatial clustering identification.}  \textbf{G.} and \textbf{P.} refer to graph-based modality (transcriptomics) and path-based modality (WSIs), respectively. Best performance in \textbf{bold}, second best \underline{underlined}. The standard deviation is reported over five runs and evaluated using the ARI metric.
}
\label{tab:results-one}
\renewcommand{\arraystretch}{1.2}  % Adjust row height
\setlength{\tabcolsep}{4pt}        % Adjust column spacing
\begin{tabular}{l|cc|>{\centering\arraybackslash}p{1.4cm} >{\centering\arraybackslash}p{1.4cm} >{\centering\arraybackslash}p{1.4cm} >{\centering\arraybackslash}p{1.4cm} >{\centering\arraybackslash}p{1.4cm} >{\centering\arraybackslash}p{1.4cm}|c}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{Modality}} & \multicolumn{6}{c|}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Overall}} \\

\cline{4-9}
 & \textbf{G.} & \textbf{P.} & 151508 & 151509 & 151510 & 151673 & 151675 & 151676 & \\
\hline

CTransPath & & $\checkmark$ & 0.0544 & 0.1093 & 0.1028 & 0.1664 & 0.1908 & 0.1078 & 0.1219 \\
& & & \scriptsize(± 0.003) & \scriptsize(± 0.009) & \scriptsize(± 0.011) & \scriptsize(± 0.005) & \scriptsize(± 0.034) & \scriptsize(± 0.039) &  \\

UNI & & $\checkmark$ & 0.2037 & 0.1522 & 0.1558 & \underline{0.1939} & 0.2018 & \underline{0.1668} & 0.1790 \\
& & & \scriptsize(± 0.008) & \scriptsize(± 0.009) & \scriptsize(± 0.006) & \scriptsize(± 0.014) & \scriptsize(± 0.014) & \scriptsize(± 0.012) &  \\

Prov-GigaPath & & $\checkmark$ & 0.0883 & 0.1164 & 0.0966 & 0.1531 & 0.1764 & 0.1303 & 0.1269 \\
& & & \scriptsize(± 0.003) & \scriptsize(± 0.004) & \scriptsize(± 0.022) & \scriptsize(± 0.019) & \scriptsize(± 0.023) & \scriptsize(± 0.022) &  \\

Hibou & &$\checkmark$ & 0.0526 & 0.0730 & 0.0598 & 0.1533 & 0.1903 & 0.1056 & 0.1057 \\
& & & \scriptsize(± 0.001) & \scriptsize(± 0.026) & \scriptsize(± 0.021) & \scriptsize(± 0.024) & \scriptsize(± 0.039) & \scriptsize(± 0.002) &  \\

CONCH & & $\checkmark$ & 0.1036 & 0.1576 & 0.1684 & 0.1610 & 0.2061 & 0.1263 & 0.1538 \\
& & & \scriptsize(± 0.023) & \scriptsize(± 0.050) & \scriptsize(± 0.042) & \scriptsize(± 0.007) & \scriptsize(± 0.021) & \scriptsize(± 0.045) &  \\

Scanpy & $\checkmark$ & & 0.0451 & 0.0601 & 0.0344 & 0.1165 & 0.1192 & 0.1069 & 0.0804 \\
& & & \scriptsize(± 0.029) & \scriptsize(± 0.015) & \scriptsize(± 0.000) & \scriptsize(± 0.004) & \scriptsize(± 0.002) & \scriptsize(± 0.000) &  \\

scFoundation & $\checkmark$ & & 0.1731 & \textbf{0.3557} & 0.1351 & 0.1393 & 0.1290 & 0.1178 & 0.1750 \\
& & & \scriptsize(± 0.032) & \scriptsize(± 0.027) & \scriptsize(± 0.058) & \scriptsize(± 0.009) & \scriptsize(± 0.018) & \scriptsize(± 0.009) &  \\

scGPT & $\checkmark$ &  & 0.1507 & 0.2192 & \textbf{0.2252} & 0.1197 & 0.1183 & 0.1051 & 0.1563 \\
& & & \scriptsize(± 0.043) & \scriptsize(± 0.104) & \scriptsize(± 0.006) & \scriptsize(± 0.017) & \scriptsize(± 0.032) & \scriptsize(± 0.002) &  \\

CLIP & $\checkmark$ & $\checkmark$ & \underline{0.2252} & 0.1931 & 0.1154 & 0.1191 & 0.2020 & 0.1494 & 0.1674 \\
& & & \scriptsize(± 0.001) & \scriptsize(± 0.021) & \scriptsize(± 0.001) & \scriptsize(± 0.002) & \scriptsize(± 0.001) & \scriptsize(± 0.003) &  \\

PLIP & $\checkmark$ & $\checkmark$ & \textbf{0.2299} & 0.1612 & \underline{0.1764} & 0.1537 & 0.1702 & 0.1358 & 0.1712 \\
& & & \scriptsize(± 0.002) & \scriptsize(± 0.001) & \scriptsize(± 0.021) & \scriptsize(± 0.025) & \scriptsize(± 0.013) & \scriptsize(± 0.016) &  \\

\hline

ST-Align \scriptsize(zero-shot) & $\checkmark$ & $\checkmark$ & 0.1923 & 0.2667 & 0.1544 & 0.1879 & \underline{0.2663} & \underline{0.1887} & \underline{0.2094} \\
& & & \scriptsize(± 0.001) & \scriptsize(± 0.012) & \scriptsize(± 0.020) & \scriptsize(± 0.014) & \scriptsize(± 0.023) & \scriptsize(± 0.005) &  \\

ST-Align \scriptsize(few-shot) & $\checkmark$ & $\checkmark$ & 0.2047 & \underline{0.2927} & 0.1276 & \textbf{0.2304} & \textbf{0.2729} & \textbf{0.1960} & \textbf{0.2207} \\
& & & \scriptsize(± 0.005) & \scriptsize(± 0.017) & \scriptsize(± 0.021) & \scriptsize(± 0.011) & \scriptsize(± 0.019) & \scriptsize(± 0.034) &  \\

% ST-Align & $\checkmark$ & $\checkmark$ & \textbf{0.2955} & \textbf{0.4346} & \textbf{0.4044} & \textbf{0.2935} & \textbf{0.3201} & \textbf{0.2135} & \textbf{0.3269} \\
\hline
\end{tabular}
\end{table*}
